Imagine-2-Drive: Leveraging High-Fidelity World Models via Multi-Modal Diffusion Policies

World Model-based Reinforcement Learning (WMRL) enables sample efficient policy learning by reducing the need for online interactions which can potentially be costly and unsafe, especially for autonomous driving. However, existing world models often suffer from low prediction fidelity and compounding one-step errors, leading to policy degradation over long horizons. Additionally, traditional RL policies, often deterministic or single Gaussian-based, fail to capture the multi-modal nature of decision-making in complex driving scenarios. To address these challenges, we propose Imagine-2-Drive, a novel WMRL framework that integrates a high-fidelity world model with a multi-modal diffusion-based policy actor. It consists of two key components: DiffDreamer, a diffusion-based world model that generates future observations simultaneously, mitigating error accumulation, and DPA (Diffusion Policy Actor), a diffusion-based policy that models diverse and multi-modal trajectory distributions. By training DPA within DiffDreamer, our method enables robust policy learning with minimal online interactions. We evaluate our method in CARLA using standard driving benchmarks and demonstrate that it outperforms prior world model baselines, improving Route Completion and Success Rate by 15% and 20% respectively.

==> 01_intro.tex <==
\section{INTRODUCTION}\label{sec:introduction}

Autonomous driving systems must operate safely and effectively in complex, dynamic environments, where accurate prediction of future events and diverse behavioral modeling are critical for informed decision-making. The ability to foresee potential obstacles, navigate uncertain traffic conditions, and make proactive adjustments to driving strategies relies on robust future state prediction capabilities, which is especially challenging in the image state space.

\begin{figure}[!h]
    \centering
    \includegraphics[width=1\linewidth]{images/column_teaser.jpg}
    \caption{\textbf{Iterative Training of \textit{DPA} and \textit{DiffDreamer}:} Both the modules are trained iteratively while the other module is kept frozen. To train the \textit{DiffDreamer}, data tuples which are collected from a frozen \textit{DPA} rollouts in the simulator are sampled from replay buffer which are used to compute $\nabla_{\phi}\mathcal{L}_{WM}$. To train \textit{DPA}, it is rolled out in a frozen \textit{DiffDreamer} from which $\nabla_{\theta}\bar{\mathcal{J}}_{RL}$ is computed. This process is iteratively repeated to keep both \textit{DPA} and \textit{DiffDreamer} in sync with each other.}
    \label{fig:iterative_training}
\end{figure}


World model-based Reinforcement Learning approaches \cite{pan2022isodreamisolatingleveragingnoncontrollable, li2024think2driveefficientreinforcementlearning} have emerged as a promising solution to this challenge by simulating future states based on current observations and actions. These models enable autonomous vehicles (AVs) to internally “imagine” possible future scenarios, facilitating more efficient exploration and reducing the risks and costs associated with real-world interactions. The significant advantages of world models also highlights the importance of learning an accurate world model. However, the utility of these world models is often limited by the nature of traditional RL policies. Most RL policies are constrained to deterministic outputs or single gaussian distributions, which fail to capture the full range of possible behaviors. This undermines the adaptability of the world models and their ability to handle the complexity and variability found in driving environments.


Current WMRL \cite{hafner2020dreamcontrollearningbehaviors, hafner2022masteringataridiscreteworld, hafner2024masteringdiversedomainsworld, pan2022isodreamisolatingleveragingnoncontrollable, deng2021dreamerproreconstructionfreemodelbasedreinforcement} approaches, model the environment dynamics in latent space using a Recurrent State Space Model (RSSM) \cite{hafner2019learninglatentdynamicsplanning} based network. A common limitation of these approaches is their reliance on single-step transition models, where errors accumulate over multi-step planning, causing planned states to drift from the on-policy distribution. Prior works \cite{wang2023drivedreamerrealworlddrivenworldmodels, ding2024diffusionworldmodelfuture, gao2024vistageneralizabledrivingworld} leverage video diffusion \cite{blattmann2023stablevideodiffusionscaling} based approaches to predict the future states simultaneously, with \textit{VISTA} \cite{gao2024vistageneralizabledrivingworld} being the most versatile and accurate.

To overcome these limitations, we present \textbf{\notcool}, a novel framework that incorporates two key innovations: \textit{DiffDreamer}, a high-fidelity world model designed for precise future prediction, and \textit{DPA}, a diffusion-based policy actor that models diverse behavioral modes for trajectory planning. VISTAPlan extends upon the VISTA's prediction capabilities by incorporating additional modules to predict reward. These enhancements enable VISTAPlan to function as a comprehensive world model, facilitating more sample efficient planning and decision-making.

% the simulation and evaluation of trajectories generated by DPA, while DPA, trained using Denoising Diffusion Policy Optimization (DDPO), leverages its ability to generate multi-modal action distributions.
Similar to \cite{janner2022planningdiffusionflexiblebehavior, saha2023edmpensembleofcostsguideddiffusionmotion, ze20243ddiffusionpolicygeneralizable, jiang2023motiondiffusercontrollablemultiagentmotion, yang2024diffusionesgradientfreeplanningdiffusion}, \textit{DPA} utilizes a diffusion based model to predict the trajectory (a sequence of actions) in a single pass.
Being a generative model, it allows \textit{DPA} to model multiple behavioral modes.
By incorporating the diverse behavior patterns inherent to diffusion policies, our framework can explore a broader range of behaviors, thereby improving its overall performance and robustness. \textit{DPA} is trained with PPO \cite{schulman2017proximalpolicyoptimizationalgorithms} using \textit{DiffDreamer} to simulate and evaluate trajectories to maximize the episodic return.

We validate our framework in the autonomous driving domain in CARLA \cite{dosovitskiy2017carlaopenurbandriving} simulator, demonstrating its superiority over existing methods. A comprehensive evaluation across diverse driving scenarios highlights the contributions of each component, and how they effectively complement one another to enhance the overall performance.

% To summarize, our key contributions are:
% \begin{enumerate}
%     \item We propose VISTAPlan, a high fidelity world model based reinforcement learning framework for autonomous driving, with image as the sole input modality. VISTAPlan extends VISTA by incorporating additional reward and discount factor heads enabling
%     it for effective planning and decision-making.

%     \item DPA, a novel diffusion based policy actor which can model multiple behavioral modes, thereby enabling it to explore a broader range of behaviors. It is trained using DDPO to maximize the cumulative sum of rewards over trajectories.

%     \item Thorough analysis of our approach and baselines in complex CARLA driving scenarios over standard driving metrics to understand the effectiveness of our framework and validating each component.
% \end{enumerate}

To summarize, our key contributions include:
\begin{enumerate}
    % \item We propose VISTAPlan, a high fidelity video-diffusion based world model for model based reinforcement learning, with image as the sole input modality. The efficacy of our world model is shown in Table \ref{table:FIDandFVD} and Table \ref{table:Ablation-Driving-metrics} where we compare with other RSSM based world models, which highlights the effects of model accuracy.

    % \item We propose VISTAPlan, a high-fidelity video-diffusion based world model for model-based reinforcement learning, with image as the sole input modality. The effectiveness of VISTAPlan is demonstrated in Table \ref{table:FIDandFVD} and Table \ref{table:Ablation-Driving-metrics}, where we compare it against RSSM-based world models, which highlights the impact of improved prediction fidelity and model accuracy.

    % \item We introduce DPA, a diffusion policy actor which can model multiple behavioral modes, enabling it to explore a broader range of behaviors. The effectiveness of 

    % \item We propose DPA, a novel diffusion based policy actor which can model multiple behavioral modes, enabling it to explore a broader range of behaviors. The efficacy 

    \item \textbf{High-fidelity video-diffusion based world model:} We propose the use of video diffusion models for MBRL, operating solely on image inputs. Unlike traditional RSSM-based single-step world models, our approach achieves superior prediction fidelity and model accuracy, as demonstrated through comprehensive comparisons in Tables \ref{table:FIDandFVD} and \ref{table:Ablation-Driving-metrics}.

    \item \textbf{Multi-Modal Diffusion Policy Actor:} We introduce a diffusion-based policy trained using PPO \cite{schulman2017proximalpolicyoptimizationalgorithms} that can effectively model and generate diverse behavioral modes in policy learning. This approach addresses the fundamental challenge of capturing multiple distinct behavioral patterns within a single policy architecture, demonstrating superior performance over single-Gaussian policies as evidenced in Table \ref{table:Ablation-Driving-metrics}.

    \item Our extensive evaluation on CARLA driving tasks demonstrates that our framework outperforms both existing model-based approaches \cite{pan2022isodreamisolatingleveragingnoncontrollable, hafner2024masteringdiversedomainsworld} and model-free baselines \cite{mnih2013playingatarideepreinforcement, schulman2017proximalpolicyoptimizationalgorithms} across standard driving metrics, with all methods using image as the sole input modality.
\end{enumerate}

==> 03_methodology_old.tex <==
\section{METHODOLOGY} \label{methodology}

\notcool is a World Model based RL framework designed for long-horizon trajectory planning using only front-facing camera image as input. The framework aims to generate a collision-free trajectory over a prediction horizon $H$, based on a sequence of past and current observations.

As depicted in Fig. 2, the framework consists of three key components:
\begin{enumerate}
    \item \textbf{State Encoder:} Encodes the sequence of $P$ past front-view RGB camera observations, together with the current observation, to provide contextual information for current state.
    \item \textbf{VISTAPlan:} A high-fidelity world model that facilitates efficient planning by accurately predicting future observations.
    \item \textbf{DPA:} A diffusion based policy actor to produce a trajectory of actions which maximizes the cumulative sum of rewards over the prediction horizon $H$.
\end{enumerate}

\textbf{Notation:} This paper differentiates between two categories
of timesteps: diffusion timesteps, indicated by superscripts
$k \in \{1, \dots, T\}$, and environment timesteps, denoted by subscripts $t \in \{1, \dots, N\}$.

\subsection{\textbf{Approximate POMDP with MDP}}
Using a single frame as the state in autonomous driving lacks the necessary temporal context to capture object motion and changes over time. This limitation makes it challenging to formulate the problem as a Markov Decision Process (MDP), which assumes that the current state captures all relevant information for decision-making. To address this, we approximate an MDP by incorporating a sequence of previous observations, thereby adding temporal information to the state representation. This approach effectively transforms the problem from a POMDP to an MDP by including a fixed-length history, which provides a richer context for understanding the dynamics of the driving environment.

Following ViNT \cite{shah2023vintfoundationmodelvisual}, we use a \textit{State Encoder} which tokenize each observation image $\{o_{i}\}_{t-P}^{t}$ into an embedding of size $d_{model} = 512$ with an EfficientNet-B0 \cite{tan2020efficientnetrethinkingmodelscaling} model which outputs a feature vector $\zeta(o_{i})$. The individual tokens are then combined with a positional encoding and fed into a transformer backbone $\mathcal{F}_{sa}$. We use a decoder-only transformer with $n_{L}=4$ multi-headed attention blocks, each with $n_{H}=4$ heads and $d_{FF}=2048$ hidden units. The output tokens are concatenated and flattened, then passed through MLP layers to give a final state embedding $s_{t} \in \mathbb{R}^{32}$
\begin{subequations}
    \begin{gather}
        s_{t} = MLP \left( \mathcal{F}_{sa} \left( \zeta(o)_{t-P:t} \right) \right) \label{state-encoder}
    \end{gather}
\end{subequations}


% \subsection{\textbf{VISTAPlan}}
% We leverage VISTA's high-fidelity prediction capabilities as the foundation for building our world model. Given the $P$ past and current observations $\{o_{i}\}_{t-P}^{t}$, we predict $H$ future observations $\{o_{i}\}_{t+1}^{t+H}$ conditioned on a action trajectory $\tau \in \mathbb{R}^{H \times 2}$. 

% \textbf{Fourier Trajectory Encoding:} The trajectory is encoded using the Fast Fourier Transform (FFT) \cite{mildenhall2020nerfrepresentingscenesneural} which offers a compact frequency-domain representation that captures the trajectory's underlying patterns.
% \begin{subequations}
%     \begin{gather}
%         \tau_{t} = \left( a_{t}, a_{t+1}, \dots, a_{t+H} \right) \label{Trajectory_representation} \\
%         c_{t} = FFT \left( \tau_{t} \right) \label{trajectory-encoder}
%     \end{gather}
% \end{subequations}

% \textbf{Future State Prediction:} To predict the future observations $\{o_{i}\}_{t+1}^{t+H}$ corresponding to $\tau_{t}$, we use the Stable Video Diffusion model (SVD) \cite{blattmann2023stablevideodiffusionscaling} used in VISTA.
% \begin{subequations}
%     \begin{gather}
%         o_{t+1:t+H} = SVD(o_{t-P:t}, c_{t}) \label{svd-equation}
%     \end{gather}
% \end{subequations}
% Using the state encoder \ref{state-encoder} and $\{o_{i}\}_{t+1}^{t+H}$, we can get future states $\{s_{i}\}_{t}^{t+H}$.
% This capability allows the model to anticipate the future state of the environment dependent on the trajectory, which is crucial for safe and effective decision making in complex driving scenarios.

% \vspace{5px}
% \textbf{Additional Required MDP Components:} To use VISTA as a world model, we add additional sub-modules to predict future rewards $\hat{r}_{t}$ and $\hat{\gamma}_{t}$ using $s_{t}$ and $a_{t}$

% \begin{equation}
% \hat{r}_{t} \sim p_{\phi}\left( \hat{r}_{t} \mid s_{t}, a_{t} \right), \quad \hat{\gamma}_{t} \sim p_{\phi}\left( \hat{\gamma}_{t} \mid s_{t}, a_{t} \right)
% \label{eq:reward-gamma-predict}
% \end{equation}

% This provides us with all the components required for MDP and to use VISTAPlan as a world model for planning.

% \textbf{Loss Function:} In addition to VISTA's loss function $\mathcal{L}_{VISTA}$ defined in equation 6 of \cite{gao2024vistageneralizabledrivingworld}, we add the additional loss functions for learning reward to get a final loss function $\mathcal{L}_{WM}$:
% \begin{equation}
% \begin{aligned}
%     \mathcal{L}_{WM} = \mathcal{L}_{Vista} - 
%     \mathbb{E}_{\tau \sim p(\tau \mid \pi)} \Bigg[ \sum_{t=1}^{H} &\ln p_{\phi}\left( \hat{r}_{t} \mid s_{t}, a_{t} \right) + \\
%     & \ln p_{\phi}\left( \hat{\gamma}_{t} \mid s_{t}, a_{t} \right) \Bigg] \label{DDPO-IS}
% \end{aligned}
% \end{equation}




% \subsection{\textbf{Diffusion Policy Actor (DPA)}}
% Given the current state $s_{t}$, we use a diffusion based policy network $(\pi_{\theta})$ to predict the trajectory $\tau_{t}$ \ref{Trajectory_representation}. The diffusion model captures complex, multi-modal action distributions, enabling effective long-horizon planning essential for autonomous driving.

% However, unlike imitation learning, where diffusion policies are trained with fixed datasets of expert actions, our RL setting lacks predefined targets. Instead, the policy learns to maximize cumulative rewards through exploration and interaction with the environment.

% The reinforcement learning (RL) objective is for the agent to maximize $\mathcal{J}_{RL}(\pi)$, the expected cumulative reward over trajectories sampled from its policy.

% \textit{Without losing generalizibility, we assume the current environment timestep (t) to be 0}.
% \begin{equation}
% \begin{aligned}
%     \mathcal{J}_{RL}(\pi) = \mathbb{E}_{\tau \sim \textit{p}_{\theta}(\tau \mid \pi)} \biggl[ \sum_{t=1}^{H}\hat{\gamma}_{t} \hat{r}_{\phi}(s_{t}, a_{t}) \biggr] \label{RL}
% \end{aligned}
% \end{equation}

% Following DDPO \cite{black2024trainingdiffusionmodelsreinforcement}, we formulate the policy denoising process as an MDP itself and use policy gradients method to train the DPA.

% We begin with a randomly initialized diffusion policy network. Sampling from the policy network begins with a noisy trajectory sample drawn from  a isotropic gaussian distribution, $\tau^{T} \sim \mathcal{N(\textbf{0, $\sigma^{2}$I})}$. The reverse process is defined by a learned distribution $p_{\theta}(\tau^{k-1} | \tau^{k}, s_{0})$, which progressively ``denoises" the action sequence to produce a sequence of trajectories $\{ \tau^{T}, \tau^{T-1}, \dots, \tau^{0} \}$ ending with the sample $\tau^{0}$.

% After getting the final denoised trajectory $\tau^{0}$, given current state $s_{t}$, we query our world model to get future states $\{s_{i}\}_{t=1}^{H}$ using \ref{svd-equation} and \ref{state-encoder}.

% \textbf{Denoising as a multi-step MDP:} In our formulation, the denoising process itself is viewed as an MDP where:
% \begin{subequations}
%     \begin{gather}
%         s_{DDPO}^{k} = (\tau^{k}, s_{0}) \label{state_ddpo} \\
%         a_{DDPO}^{k} = \tau^{k-1} \label{action_ddpo} \\
%         r^{k}_{DDPO} =
%         \begin{cases} 
%         \sum_{t=1}^{H}\hat{\gamma}_{t} \hat{r}_{\phi}(s_{t}, a_{t}) & \text{if } k = 0 \\
%         0 & \text{otherwise}
%         \end{cases} \label{crtic-equation} \\
%         \pi_{DDPO}(a_{DDPO}^{k} \mid s^{k}_{DDPO}) = p_{\theta}(\tau^{k-1} | \tau^{k}, s_{0})
%     \end{gather}
% \end{subequations}

% \textbf{Denoising Diffusion RL Objective:} The objective for this MDP $\mathcal{J}_{DDRL}(\theta)$ is to maximize the reward signal $r_{DDPO}$.
% \begin{equation}
% \begin{aligned}
%     \mathcal{J}_{DDRL}(\theta) = \mathbb{E}_{\textbf{$s_{0}$} \sim \textit{p}(s_{0}), \tau^{0} \sim \textit{p}_{\theta}(\tau^{0} \mid s_{0})} \biggl[ p_{\theta}(r^{0}_{DDPO} \mid \tau^{0}) \biggr] \label{DDRL}
% \end{aligned}
% \end{equation}

% This formulation further enables the estimation of policy gradients. With access to both likelihood and gradients of likelihood, we follow the formulation in \cite{black2024trainingdiffusionmodelsreinforcement, fan2023optimizingddpmsamplingshortcut} to make direct Monte Carlo estimates of $\nabla_{\theta}\mathcal{J}_{DDRL}$, by sampling, and then performing parameter update. We adopt the importance sampling estimator \cite{1617243} and substitute the per-step return with the final reward $r^{0}_{DDPO}$.
% \begin{equation}
% \begin{aligned}
%     \nabla_{\theta}\mathcal{J}_{DDRL} &= \mathbb{E} \Biggl[ \sum_{k=0}^{T} \frac{\textit{p}_{\theta}(\tau^{k-1} | \tau^{k}, s_{0}) \,}{\textit{p}_{\theta_{old}}(\tau^{k-1} | \tau^{k}, s_{0}) \,} \\
%     & \quad \times \nabla_{\theta} \log \textit{p}_{\theta}(\tau^{k-1} | \tau^{k}, s_{0}) \, r^{0}_{DDPO} \Biggr] \label{DDPO-IS}
% \end{aligned}
% \end{equation}

% in which the expectation is taken over the trajectories sampled with $p_{\theta_{old}}$, i.e., the previous sampler. The estimator becomes less accurate if $p_{\theta_{old}}$ deviates too much from $p_{\theta}$. We adopt the trust region \cite{schulman2017trustregionpolicyoptimization} for regularizing the change of $\theta$ w.r.t $\theta_{old}$, which in practice we adopt the clipping proposed in proximal policy optimization \cite{schulman2017proximalpolicyoptimizationalgorithms}.

% This procedure effectively trains the diffusion policy network to 
% generate high reward action-sequences $(\tau)$ that maximize cumulative rewards, improving autonomous driving performance.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm}
% \caption{Placeholder for Psuedo-Code}\label{alg:cap}
% \begin{algorithmic}
% \Require $n \geq 0$
% \Ensure $y = x^n$
% \State $y \gets 1$
% \State $X \gets x$
% \State $N \gets n$
% \While{$N \neq 0$}
% \If{$N$ is even}
%     \State $X \gets X \times X$
%     \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
% \ElsIf{$N$ is odd}
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
% \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{\textbf{VISTAPlan}}
Stable Video Diffusion (SVD) models have demonstrated high-fidelity and frame consistency by leveraging spatiotemporal denoising and cross-frame attention mechanisms. These models ensure smooth temporal transitionns while preserving fine-grained details. By capturing long-range dependencies and enforcing structural coherence, they can generate realistic, high-resolution video sequences with consistent motion dynamics. 

To overcome the issues of compounding errors and low-fidelity, typically found in one-step prediction RSSM-based world models, we leverage SVD as the foundation for building our world model to predict multiple future observations at once. Given the $P$ past and current observations $\{o_{i}\}_{t-P}^{t}$, we predict $H$ future observations $\{o_{i}\}_{t+1}^{t+H}$ conditioned on a action trajectory $\tau \in \mathbb{R}^{H \times 2}$. \newline
% \newline

% \textbf{Fourier Trajectory Encoding:} The trajectory $\tau$ is encoded using the Fast Fourier Transform (FFT) \cite{mildenhall2020nerfrepresentingscenesneural} which offers a compact frequency-domain representation that captures the trajectory's underlying patterns.
% \begin{subequations}
%     \begin{gather}
%         \tau_{t} = (a_{t}, a_{t+1}, \dots, a_{t+H}) \\
%         c_{t} = FFT(\tau_{t})
%     \end{gather}
% \end{subequations}

\textbf{Fourier Trajectory Encoding:} To effectively encode the trajectory $\tau$, we apply a fourier embedding (FFT) \cite{mildenhall2020nerfrepresentingscenesneural}, which transforms the raw spatial coordinates into a frequency domain representation. This embedding captures both low and high-frequency components, allowing the model to represent smooth and periodic motion patterns more effectively.
\begin{subequations}
    \begin{gather}
        \tau_{t} = (a_{t}, a_{t+1}, \dots, a_{t+H}) \\
        c_{t} = FFT(\tau_{t})
    \end{gather}
\end{subequations}

\textbf{Future State Prediction:} To predict the future observations $\{o_{i}\}_{t+1}^{t+H}$ corresponding to $\tau_{t}$, while enforcing dynamic consistency with respect to position, velocity and acceleration, we replace the first $P+1$ noisy frames of the SVD model with the past $P$ and current observations $\{o_{i}\}_{t-P}^{t}$. This approach grounds the model's predictions in accurate initial conditions and reducing drift.
\begin{subequations}
    \begin{gather}
        o_{t+1:t+H} = SVD(o_{t-P:t}, c_{t})
    \end{gather}
\end{subequations}
Using the state encoder \ref{state-encoder} and $\{o_{i}\}_{t+1}^{t+H}$, we can get the corresponding states $\{s_{i}\}_{t+1}^{t+H}$. This capability allows the model to accurately predict the future states of the environment dependent on the trajectory, which is crucial for sample efficient and safe decision making. \newline

\textbf{Additional Required MDP Components:} To employ VISTAPlan as a world model, we integrate additional sub-modules to predict future rewards $r_{t}$ and discount factors $\gamma(t)$ based on the state $s_{t}$ and action $a_{t}$, thereby completing the Markov Decision Process (MDP) formulation, enabling effective policy optimization.
\begin{equation}
\hat{r}_{t} \sim p_{\phi}\left( \hat{r}_{t} \mid s_{t}, a_{t} \right), \quad \hat{\gamma}_{t} \sim p_{\phi}\left( \hat{\gamma}_{t} \mid s_{t}, a_{t} \right)
\label{eq:reward-gamma-predict}
\end{equation}

\textbf{Loss Function:} For future frame predictions, in addition to usual noise reconstruction loss $\mathcal{L}_{diffusion}$, we incorporate two additional losses $\mathcal{L}_{dynamics}$ and $\mathcal{L}_{structure}$ from section 3.1 of \cite{gao2024vistageneralizabledrivingworld} for enhanced frame prediction:
\begin{enumerate}
    \item \textit{Dynamics Enhancement Loss} $\mathcal{L}_{dynamics}$: focuses on accurately capturing the motion dynamics of objects within the generated videos. This loss encourages the model to learn realistic movement patterns, ensuring that the generated sequences maintain coherence over time.
    \item \textit{Structure Preservation Loss} $\mathcal{L}_{structure}$: reinforces the structural integrity of the generated scenes. By emphasizing the preservation of spatial relationships and object configurations, this loss helps in producing videos that are not only visually appealing but also contextually accurate.
\end{enumerate}
The combined loss function for training the SVD model $\mathcal{L}_{SVD}$ becomes:
\begin{equation}
    \mathcal{L}_{SVD} = \mathcal{L}_{diffusion} + \lambda_{1} \mathcal{L}_{dynamics} + \lambda_{2} \mathcal{L}_{structure} \label{SVD_loss_function}
\end{equation}
For a detailed overview of the loss functions used in $\mathcal{L}_{SVD}$, interested readers are encouraged to refer to section 3.1 of \cite{gao2024vistageneralizabledrivingworld}.

To train the additional reward and discount prediction heads, we add two additional losses to get the final world model loss $\mathcal{L}_{WM}$:
\begin{equation}
\begin{aligned}
    \mathcal{L}_{r} = \mathbb{E}_{\tau \sim p(\tau \mid \pi)} \Bigg[ \sum_{t=1}^{H} &\ln p_{\phi}\left( \hat{r}_{t} \mid s_{t}, a_{t} \right) \Bigg] \\
    \mathcal{L}_{WM} = \mathcal{L}_{SVD} + \lambda_{3} \mathcal{L}_{r}
\end{aligned}
\end{equation}

Here $\lambda_{1}$, $\lambda_{2}$ and $\lambda_{3}$ are hyperparameters to balance the weights of the losses in the final world model loss function $\mathcal{L}_{WM}$.

% \subsection{\textbf{Diffusion Policy Actor (DPA)}}
% \dpa is a policy $\pi_{\theta}$ parameterized by a DDPM which takes in $s$ as a conditioning argument, and parameterizes $p_{\theta}(a^{k-1} \mid a^{k}, s)$. Aligning with the common practice, we predict an action chunk $(a_{t:t+H})$, $H$ future actions, where $H$ is the prediction horizon.

% \textbf{Denoising as a multi-step MDP:} As shown in \cite{black2024trainingdiffusionmodelsreinforcement}, we formulate the denoising process as a multi-step MDP. We begin with a randomly initialized diffusion policy network. Sampling from the policy network begins with a noisy trajectory sample drawn from a isotropic Gaussian distribution, $\tau^{T}_{t} \sim \mathcal{N(\textbf{0, $\sigma^{2}$I})}$. The reverse process is defined by a learned distribution $p_{\theta}(\tau^{k-1}_{t} | \tau^{k}_{t}, s_{t})$, which progressively ``denoises" the action sequence to produce a sequence of trajectories $\{ \tau^{T}_{t}, \tau^{T-1}_{t}, \dots, \tau^{0}_{t} \}$ ending with the sample $\tau^{0}_{t}$.

% Without losing generalizibility, we assume the  current environment timestep (t) to be 0 and define the Diffusion MDP as:
% \begin{subequations}
%     \begin{gather}
%         s_{DDPO}^{k} = (\tau^{k}, s_{0}) \label{state_ddpo} \\
%         a_{DDPO}^{k} = \tau^{k-1} \label{action_ddpo} \\
%         r^{k}_{DDPO} =
%         % \begin{cases} 
%         % \sum_{t=1}^{H}\hat{\gamma}_{t} \hat{r}_{\phi}(s_{t}, a_{t}) & \text{if } k = 0 \\
%         % 0 & \text{otherwise}
%         % \end{cases} \label{crtic-equation} \\
%         \begin{cases} 
%         \hat{r}_{\phi}(s_{0}, a_{0}^{k}) & \text{if } k = 0 \\
%         0 & \text{otherwise}
%         \end{cases} \label{crtic-equation} \\
%         \pi_{DDPO}(a_{DDPO}^{k} \mid s^{k}_{DDPO}) = p_{\theta}(\tau^{k-1} | \tau^{k}, s_{0}) \\
%         % p_{\theta}(\tau^{k-1} | \tau^{k}, s_{0}) = \mathcal{N}(\tau^{k-1}; \mu(\tau^{k}), \varepsilon_{\theta}(\tau^{k}, k, s_{0}))
%         p_{\theta}(\tau^{k-1} \mid \tau^{k}, s_{0}) = \mathcal{N}(\tau^{k-1}; \mu(\tau_{k}, \varepsilon_{\theta}(\tau^{k}, k, s_{0})), \sigma^{2}I) \label{dpa_gaussian}
%     \end{gather}
% \end{subequations}
% % from Eq. \ref{dpa_gaussian}, we can analytically get the log-likelihood of the $\pi_{DDPO}(a_{DDPO}^{k} \mid s^{k}_{DDPO})$ for policy gradient updates.

% \textbf{Denoising Diffusion RL Objective:} The objective for the environment MDP is to maximize the a discounted cummulative reward defined as:
% \begin{subequations}
%     \begin{gather}
%         \mathcal{J} = \mathbb{E}_{s_{0} \sim p(s_{0})} \biggl[ \sum_{t \geq 0} \gamma(t)R(s_{t}, a_{t}) \biggr] \label{DDRL}
%     \end{gather}
% \end{subequations}

% \begin{subequations}
%     \begin{gather}
%         \nabla_{\theta} \mathcal{J}(\pi_{\theta}) = \mathbb{E} \biggl[ \sum_{t \geq 0} \nabla_{\theta}log(p_{\theta}(\tau_{t}^{k-1} \mid \tau_{t}^{k}, s_{t}))  \biggr]
%     \end{gather}
% \end{subequations}

\subsection{\textbf{Diffusion Policy Actor (DPA)}}
WRITE IN BRIEF WHY DIFFUSION POLICY IS USEFUL COMPARED TO REGULAR POLICIES  \newline
We use a diffusion based policy network $\pi_{\theta}$ to predict a sequence of action ($\tau_{t} = \{a_{i}\}_{t}^{t+H}$) conditioned on the current state $s_{t}$. 

However, unlike behavioral cloning methods where diffusion policies can be optimized to fit the conditional noise prediction $\varepsilon_{\theta}(\tau_{t}^{k}, s_{t}, k)$, our RL setting lacks predefined target trajectories to supervise upon. Instead, the policy learns to maximize the cummulative sum of rewards objective $\mathcal{J}_{RL}

(\pi_{\theta})$.
\begin{equation}
    \mathcal{J}_{RL}(\pi_{\theta}) = \mathbb{E}_{\tau \sim p_{\theta}(\tau | \pi_{\theta})} \biggl[\sum_{t \geq 0} r(s_{t}, a_{t}) \biggr]
\end{equation}

WRITE ABOUT FORMULATING DENOISING PROCESS AS AN MDP \newline
We begin with a randomly initialized diffusion policy network. Sampling from the policy network begins with a noisy trajectory sample drawn from a isotropic Gaussian distribution, $\tau^{T}_{t} \sim \mathcal{N(\textbf{0, $\sigma^{2}$I})}$. The reverse process is defined by a learned distribution $p_{\theta}(\tau^{k-1}_{t} | \tau^{k}_{t}, s_{t})$, which progressively ``denoises" the action sequence to produce a sequence of trajectories $\{ \tau^{T}_{t}, \tau^{T-1}_{t}, \dots, \tau^{0}_{t} \}$ ending with the sample $\tau^{0}_{t}$. \newline

\textbf{Denoising as a multi-step MDP:} The Denoising MDP uses timestep $\bar{t}(t,k) = tK + (K - k - 1)$ corresponding to (\textit{t,k}), which increase in $t$. The states, actions and rewards are:
\begin{subequations}
    \begin{gather}
        \bar{s}_{\bar{t}(t,k)} = (\tau_{t}^{k+1}, s_{t}) \\
        \bar{a}_{\bar{t}(t,k)} = \tau_{t}^{k}) \\
        \bar{r}_{\bar{t}(t,k)} = \begin{cases} 
        \sum_{t=1}^{A}\gamma_{t} r(s_{t}, a_{t}) & \text{if } k = 0 \\
        0 & \text{otherwise}
        \end{cases}
    \end{gather}
\end{subequations}
We assign rewards only to the final denoising step, corresponding to actions $a_{t:t+A}^{0}$ executed after each Denoising MDP. The DPA policy $\pi_{\theta}$ parameterizes to:
% \begin{equation}
%     \bar{\pi}_{\theta}(\tau_{t}^{k} \mid \tau_{t}^{k+1}, s_{t}) = \mathcal{N}(\tau_{t}^{k}, \mu(\tau_{t}^{k}, \varepsilon_{\theta}(\tau_{t}^{k+1}, k+1, s_{t}), \sigma^{2}I))
% \end{equation}
\begin{equation}
\begin{aligned}
    \bar{\pi}_{\theta}(\bar{a}_{\bar{t}(t,k)} \mid \bar{s}_{\bar{t}(t,k)}) = \pi_{\theta}(\tau_{t}^{k} \mid \tau_{t}^{k+1}, s_{t}) \\ = \mathcal{N}(\tau_{t}^{k}, \mu(\tau_{t}^{k}, \varepsilon_{\theta}(\tau_{t}^{k+1}, k+1, s_{t}), \sigma^{2}I))
\end{aligned}
\end{equation}

\textbf{Policy Optimization:} We optimize policy DPA policy parameters $\theta$ by maximizing the policy objective $\mathcal{J}_{RL}$ using policy gradient method PPO \cite{schulman2017proximalpolicyoptimizationalgorithms}.
\begin{equation}
    \nabla_{\theta}\mathcal{J}_{RL} = \mathbb{E}_{\tau \sim \pi_{\theta}(\tau \mid s_{t})} \biggl[ \sum_{t \geq 0} \nabla_{\theta} log \pi_{\theta}() \biggr]
\end{equation}



% \setlength{\belowcaptionskip}{-15pt}
\begin{figure*}[!t]
    \centering
    \includegraphics[width=1\textwidth]{images/multi_modal_trajectory.jpg}
    \caption{\textbf{Multi-Modal Nature of \textit{DPA}:} The top-view visualization illustrates the multi-modal nature of the \textit{Diffusion-based Policy Actor (DPA)}. Starting from the same initial state, the agent follows two distinct trajectories: \textcolor{Blue}{Left} (in blue) and \textcolor{Red}{Right} (in red), generated using different random seeds. The corresponding predicted future sequences for both trajectories are shown in their respective colors, highlighting \textit{DPA's} ability to model diverse behavioral modes and predict multiple plausible futures from a single state.}
    \label{multi-modal-result}
\end{figure*}
\setlength{\belowcaptionskip}{0pt}

% \setlength{\belowcaptionskip}{-15pt}
\begin{figure}[!h]
    \centering
    \includegraphics[width=1\linewidth]{images/vista_prediction.jpg}
    \caption{\textbf{\textit{VISTAPlan} Future Prediction:} Future observation predictions from the \textit{VISTAPlan World Model}, conditioned on the input trajectory (shown in black) and current observations. Demonstrates the \textit{VISTAPlan's} ability to accurately predict future observations based on the provided context, highlighting its robust trajectory prediction capabilities.}
    \label{fig:action-controllability}
\end{figure}

==> 07_background.tex <==
\subsection{\textbf{Markov Decision Processes}}
A Markov Decision Process (MDP) is a formalization of sequential decision-making problems. An MDP is defined by a tuple $(\mathcal{S, A}, \rho_{0}, P, R)$ in which $\mathcal{S}$ is the state space, \mathcal{A} is the action space, $\rho_{0}$ is the distribution of initial states. $P$ is the transition kernel 
